Effective Delay Control in Online Network Coding

Motivated by streaming applications with stringent delay constraints, we consider the design of online network coding algorithms with timely delivery guarantees. Assuming that the sender is providing the same data to multiple receivers over independent packet erasure channels, we focus on the case of perfect feedback and heterogeneous erasure probabilities. Based on a general analytical framework for evaluating the decoding delay, we show that existing ARQ schemes fail to ensure that receivers with weak channels are able to recover from packet losses within reasonable time. To overcome this problem, we re-define the encoding rules in order to break the chains of linear combinations that cannot be decoded after one of the packets is lost. Our results show that sending uncoded packets at key times ensures that all the receivers are able to meet specific delay requirements with very high probability.

==> Makefile <==
# $Id: Makefile,v 1.3 2005/04/01 16:42:25 uid60966 Exp $
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
DVIPS = dvips
RM = rm -f

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"

MASTER = main

TEXFILES = $(wildcard *.tex *.cls *.sty)
FIGURES = $(wildcard figures/*.eps)
BIBFILES = $(wildcard *.bib)

.PHONY: clean

all:		$(MASTER).ps
# $(MASTER).pdf

%.dvi:		$(FIGURES) $(TEXFILES) $(BIBFILES)
		if test -r $*.toc; then cp $*.toc $*.toc.bak; fi
		$(LATEX) $*.tex
		egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(LATEX) $*.tex) ; true
		egrep $(RERUN) $*.log && ($(LATEX) $*.tex) ; true
		egrep $(RERUN) $*.log && ($(LATEX) $*.tex) ; true
		if cmp -s $*.toc $*.toc.bak; then echo ;else $(LATEX) $* ; fi
		$(RM) $*.toc.bak
# Display relevant warnings
		egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:		%.dvi
		dvips -t letter -Ppdf -G0 $< -o $@

%.pdf:		%.ps
		$(PDFLATEX) $<

clean:
		rm -f $(MASTER).aux $(MASTER).log $(MASTER).bbl $(MASTER).blg $(MASTER).brf \
		$(MASTER).cb $(MASTER).ind $(MASTER).idx $(MASTER).ilg $(MASTER).inx \
		$(MASTER).ps $(MASTER).dvi $(MASTER).pdf $(MASTER).toc $(MASTER).out \
		texput.log

